Scheduling Splittable Jobs on Configurable Machines

Motivated by deep neural network applications, we study the problem of scheduling splittable jobs (e.g., neural network inference tasks) on configurable machines (e.g., multi-instance GPUs). We are given $n$ jobs and a set $C$ of configurations (e.g, representing ways to configure a GPU) consisting of multisets of blocks (e.g., representing GPU instances). A schedule consists of a set of machines, each assigned some configuration in $C$ with each block in the configuration assigned to process one job. The amount of a job's demand that is satisfied by a given block is an arbitrary function of the job and block. The objective is to satisfy all demands on as few machines as possible. We provide a tight logarithmic approximation algorithm for this problem in the general setting, an asymptotic $(2 + \varepsilon)$-approximation with $O(1)$ input configurations for arbitrary $\varepsilon > 0$, and a polynomial time approximation scheme when both the number and size of configurations are $O(1)$.

==> Notes/hardness.tex <==

\noindent {\bf Hardness of approximation for combinatorial version.}
We present an approximation-preserving reduction from minimum set cover to combinatorial reconfigurable scheduling, for general $n$ and $C$.  Let ${\cal U}$ denote the set of elements and ${\cal C}$ the collection of sets in the set cover instance.  We can assume without loss of generality that there do not exist two sets $S_1$ and $S_2$ with $S_1 \subseteq S_2$, since we can eliminate $S_1$ from the set collection otherwise.  We construct an instance where each set $S$ is a configuration and each element $e$ is both a block type and a job.  The job $e$ has a unit demand, which can only be satisfied by block type $e$.  

Any set cover solution corresponds to a set of machines of same count, one machine for each set in the solution, according to the corresponding configuration; since each element is covered, it follows that each job has its unique block type included in the solution, thus satisfying the demand.  Similarly, every solution with $m$ machines corresponds to a set cover solution with $m$ sets, each corresponding to the configuration of a machine.  The $\Omega(\log n)$-hardness of approximation for the scheduling problem follows. 

\medskip
\noindent{\bf NP-hardness of approximating numerical version with all configurations allowed.}
We present a reduction from Unbounded Subset Sum to the numerical version.  Given an instance of Unbounded Subset Sum with a set $S$ of $n$ elements $0 < a_1 < a_2 < \cdots < a_n$ and target sum $k$, we construct the following instance of the numerical version.  We have one job $j$ with a demand table given by a step function with $n$ steps: for $0 \le i \le n-1$, $x \in [a_i, a_{i+1})$, $f_j(x) = a_i$ ($a_0 = 0$).  The capacity of each machine is $k$ and the demand for the job is $2k$.  

We claim that the number of machines needed for scheduling the job is two if and only if the Unbounded Subset Sum instance has a yes answer.  If the Unbounded Subset Sum instance has a yes answer, then there exists a multiset $M$ of items from $S$ whose values add up to $k$; we use two machines, each configured according to $M$, and allocate the job to each of the blocks of size corresponding to the items in $M$.  The demand table ensures that the demand of the job is satisfied.  If the demand of the job is satisfied by two machines, then each machine must serve a demand of $k$.  By the demand table, each block is of size $a_i$ for some $i$, implying the existence of a multiset $M$ of items from $S$ whose values add up to $k$.

\medskip
\noindent{\bf NP-hardness of approximating numerical version with one configuration.}
We present a reduction from Partition to the numerical version.  Given an instance of Partition with a set $S$ of $n$ elements $0 < a_1 < a_2 < \cdots < a_n$, we construct the following instance of the numerical version.  We have two jobs $j$ with a demand table given by a step function with $n$ steps: for $0 \le i \le n-1$, $x \in [a_i, a_{i+1})$, $f_j(x) = a_i$ ($a_0 = 0$).  There is exactly one configuration consisting of $n$ blocks of lengths $a_i$, $1 \le i \le n$.  The capacity of each machine is $\sum_i a_i$ and the demand for each job is $\sum_i a_i/2$.  

We claim that the number of machines needed for scheduling the job is one if and only if the Partition instance has a yes answer.  If the Partition instance has a yes answer, then there exists a way to split the $n$ blocks into two parts so that part's value adds up to $k$.  We use one machine, and assign the blocks to each job according to the Partition solution.  The demand table ensures that the demand of the job is satisfied.  If the demand of the two jobs is satisfied by one machines, then the machine serves a total demand of $\sum_i a_i$.  By the demand table, each block is of size $a_i$ for some $i$, implying the existence of a two parts of items from $S$, each part's total size adding up to $\sum_i a_i/2$.

==> Notes/superlinear.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Rectangle [id:dp558448320631086] 
\draw   (140,50) -- (140,130) -- (100,130) -- (100,50) -- cycle ;
\draw   (149.39,78.18) -- (170.61,99.39)(170.61,78.18) -- (149.39,99.39) ;
%Shape: Rectangle [id:dp752658614376557] 
\draw   (340,50) -- (340,130) -- (300,130) -- (300,50) -- cycle ;
%Shape: Rectangle [id:dp5334002244155014] 
\draw   (390,50) -- (390,130) -- (350,130) -- (350,50) -- cycle ;
%Shape: Rectangle [id:dp20571852560618442] 
\draw   (480,50) -- (480,130) -- (430,130) -- (430,50) -- cycle ;
%Shape: Rectangle [id:dp35316145341145644] 
\draw   (140,180) -- (140,260) -- (100,260) -- (100,180) -- cycle ;
%Shape: Rectangle [id:dp7437112212014001] 
\draw   (190,180) -- (190,260) -- (150,260) -- (150,180) -- cycle ;
%Shape: Rectangle [id:dp7058524269266309] 
\draw   (280,180) -- (280,260) -- (230,260) -- (230,180) -- cycle ;
%Straight Lines [id:da07490550352442416] 
\draw    (100,230) -- (140,230) ;
%Straight Lines [id:da9934640766285987] 
\draw    (150,230) -- (190,230) ;
%Straight Lines [id:da09254618934394188] 
\draw    (230,230) -- (280,230) ;

% Text Node
\draw (180,81) node [anchor=north west][inner sep=0.75pt]   [align=left] {(3x+3)};
% Text Node
\draw (108,79) node [anchor=north west][inner sep=0.75pt]   [align=left] {J{\scriptsize 1,7}};
% Text Node
\draw (309,78) node [anchor=north west][inner sep=0.75pt]   [align=left] {J{\scriptsize 2,4}};
% Text Node
\draw (51,22) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\large Fill First}};
% Text Node
\draw (51,147) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\large Optimal}};
% Text Node
\draw (358,78) node [anchor=north west][inner sep=0.75pt]   [align=left] {J{\scriptsize 3,4}};
% Text Node
\draw (401,90) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\Large ...}};
% Text Node
\draw (431,78) node [anchor=north west][inner sep=0.75pt]   [align=left] {J{\scriptsize 7x+22,4}};
% Text Node
\draw (109,198) node [anchor=north west][inner sep=0.75pt]   [align=left] {J{\scriptsize 2,4}};
% Text Node
\draw (158,198) node [anchor=north west][inner sep=0.75pt]   [align=left] {J{\scriptsize 3,4}};
% Text Node
\draw (201,220) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\Large ...}};
% Text Node
\draw (231,198) node [anchor=north west][inner sep=0.75pt]   [align=left] {J{\scriptsize 7x+22,4}};
% Text Node
\draw (109,237) node [anchor=north west][inner sep=0.75pt]   [align=left] {J{\scriptsize 1,3}};
% Text Node
\draw (159,237) node [anchor=north west][inner sep=0.75pt]   [align=left] {J{\scriptsize 1,3}};
% Text Node
\draw (244.25,237) node [anchor=north west][inner sep=0.75pt]   [align=left] {J{\scriptsize 1,3}};


\end{tikzpicture}


==> Notes/superlinear_generalized.tex <==
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Rectangle [id:dp558448320631086] 
\draw   (140,50) -- (140,130) -- (100,130) -- (100,50) -- cycle ;
\draw   (149.39,78.18) -- (170.61,99.39)(170.61,78.18) -- (149.39,99.39) ;
%Shape: Rectangle [id:dp752658614376557] 
\draw   (340,50) -- (340,130) -- (300,130) -- (300,50) -- cycle ;
%Shape: Rectangle [id:dp5334002244155014] 
\draw   (390,50) -- (390,130) -- (350,130) -- (350,50) -- cycle ;
%Shape: Rectangle [id:dp20571852560618442] 
\draw   (480,50) -- (480,130) -- (430,130) -- (430,50) -- cycle ;
%Shape: Rectangle [id:dp35316145341145644] 
\draw   (140,180) -- (140,260) -- (100,260) -- (100,180) -- cycle ;
%Shape: Rectangle [id:dp7437112212014001] 
\draw   (190,180) -- (190,260) -- (150,260) -- (150,180) -- cycle ;
%Shape: Rectangle [id:dp7058524269266309] 
\draw   (280,180) -- (280,260) -- (230,260) -- (230,180) -- cycle ;
%Straight Lines [id:da07490550352442416] 
\draw    (100,230) -- (140,230) ;
%Straight Lines [id:da9934640766285987] 
\draw    (150,230) -- (190,230) ;
%Straight Lines [id:da09254618934394188] 
\draw    (230,230) -- (280,230) ;

% Text Node
\draw (180,81) node [anchor=north west][inner sep=0.75pt]   [align=left] {J\scriptsize 1, $\frac{k-1}{2}$};
% Text Node
\draw (108,79) node [anchor=north west][inner sep=0.75pt]   [align=left] {J{\scriptsize 1,k}};
% Text Node
\draw (309,78) node [anchor=north west][inner sep=0.75pt]   [align=left] {J{\scriptsize 2, $\frac{k+1}{2}$}};
% Text Node
\draw (51,22) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\large Fill First}};
% Text Node
\draw (51,147) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\large Optimal}};
% Text Node
\draw (358,78) node [anchor=north west][inner sep=0.75pt]   [align=left] {J{\scriptsize 3, $\frac{k+1}{2}$}};
% Text Node
\draw (401,90) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\Large ...}};
% Text Node
\draw (431,78) node [anchor=north west][inner sep=0.75pt]   [align=left] {J{\scriptsize $J_{1, k}$,$\frac{k+1}{2}$}};
% Text Node
\draw (109,198) node [anchor=north west][inner sep=0.75pt]   [align=left] {J{\scriptsize 2, $\frac{k+1}{2}$}};
% Text Node
\draw (158,198) node [anchor=north west][inner sep=0.75pt]   [align=left] {J{\scriptsize 3, $\frac{k+1}{2}$}};
% Text Node
\draw (201,220) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\Large ...}};
% Text Node
\draw (231,198) node [anchor=north west][inner sep=0.75pt]   [align=left] {J{\scriptsize $J_{1, k}$,$\frac{k+1}{2}$}};
% Text Node
\draw (109,237) node [anchor=north west][inner sep=0.75pt]   [align=left] {J{\scriptsize 1, $\frac{k-1}{2}$}};
% Text Node
\draw (159,237) node [anchor=north west][inner sep=0.75pt]   [align=left] {J{\scriptsize 1, $\frac{k-1}{2}$}};
% Text Node
\draw (244.25,237) node [anchor=north west][inner sep=0.75pt]   [align=left] {J{\scriptsize 1, $\frac{k-1}{2}$}};


\end{tikzpicture}

==> knapsack_greedy.tex <==
\section{\numcms}
\label{sec:numerical}

We consider \numcms: scheduling $n$ jobs on the minimum number of configurable machines, where each job $j$ has a corresponding length $k$ demand table $\f j{}$ and demand $\d j$, and where any multiset $\sigma$ of elements in $\{1,2,\ldots,k\}$ such that $\sum_{i \in \sigma} i = k$ is a valid configuration. The main result of this section is an algorithm that produces a schedule of length $(2 +\varepsilon)\opt + 1$ for \numcms. We also provide a hardness result, showing that no polynomial-time algorithm can achieve an approximation ration better than 2, as well as preliminary results on minimizing average completion time on configurable machines. 

Our first lemma establishes hardness of approximation to better than a factor of 2 for \numcms. For a proof of Lemma~\ref{lem:numcms_hardness}, see Appendix~\ref{sec:numcms_appendix}.

\begin{lemma}
Approximating \numcms\ within an $\alpha < 2$ factor is NP-hard.%
\label{lem:numcms_hardness}
\end{lemma}

The following theorem establishes our main algorithmic result in this section. 

\begin{theorem}
    There exists an algorithm that produces a schedule of length $((2+\varepsilon) \cdot \opt) + 1$ for \numcms.
\end{theorem}
\begin{proof}
For each $j$, we define the multiset $S_j$ as the set of blocks providing the solution to the following program.
\begin{equation}
    \textstyle \min \sum_{i \in S} i \ \ \text{subject to} \ \ \sum_{i \in S} j(i) \ge d_j
\label{eq:job_knapsack}
\end{equation}
It is easy to see that executing job $j$ requires at least $\sum_{i \in S_j} i$ processing units, so $\opt \ge \frac{1}{k} \sum_j \sum_{i \in S_j} i$. Further, (\ref{eq:job_knapsack}) describes an instance of unbounded minimum knapsack, for which there exists a combinatorial FPTAS (see, e.g. \cite{JianZhao.UnboundedKnapsack.2019}). We use this FPTAS to construct sets $\hat S_j$, which entails that $(1 + \varepsilon) \opt \ge \frac{1}{k} \sum_j \sum_{i \in \hat S_j} i$. 

We then pack the blocks given by each $\hat S_j$ into maximal packings on each machine. Since all machines (except possibly one) are at least half full, the number of machines is at most $1 + \frac{2}{k} \sum_j \sum_{i \in \hat S_j} i  \le 1 + 2(1 + \varepsilon) \opt$.

We can repeat a single machine placement until we exhaust the blocks of a one size for one job, so we need at most $nk$ placements and each placement can be constructed in $O(n)$ time. So the algorithm runs in $\mathrm{poly}(n,k)$ time. 
\qed
\end{proof}


